Robust Explanation Constraints for Neural Networks

Post-hoc explanation methods are used with the intent of providing insights about neural networks and are sometimes said to help engender trust in their outputs. However, popular explanations methods have been found to be fragile to minor perturbations of input features or model parameters. Relying on constraint relaxation techniques from non-convex optimization, we develop a method that upper-bounds the largest change an adversary can make to a gradient-based explanation via bounded manipulation of either the input features or model parameters. By propagating a compact input or parameter set as symbolic intervals through the forwards and backwards computations of the neural network we can formally certify the robustness of gradient-based explanations. Our bounds are differentiable, hence we can incorporate provable explanation robustness into neural network training. Empirically, our method surpasses the robustness provided by previous heuristic approaches. We find that our training method is the only method able to learn neural networks with certificates of explanation robustness across all six datasets tested.

==> Sections/Methodology_old.tex <==
\section{Methodology}

Explanations for deep neural networks have been found to be unreliable in the face of both input and model perturbation threat models. While there is a recent line of work that aim at defending against such attacks, it is well-known that heuristic defenses are often defeated by attacks designed specifically to bypass them. Below, we state what it means for a neural network's explanation to be certifiably robust in the face of attackers. Namely, we state certification as the task of \textit{proving} that no attack can perturb the model explanation we provide.


\subsection{Bounding the Effect of Input Perturbations} 

Below we formally define what it means for an explanation $e \in \mathbb{R}^n$ to be certifiably robust.
\begin{definition} \textbf{\textit{Input-Certified Explanation}} Given a neural network $f^{\theta}$, a test input $x$, a loss function $J$, a compact input set $T$ and an error tolerance $\delta$, we say that an explanation $e$ is input certified iff: 
\begin{align}
    \forall x' \in T, \quad || e - \nabla_x J(f^{\theta}(x')) || \leq \delta
\end{align}
\end{definition}
\JH{We need the condition that the predictions of $x$ and $x'$ should be the same, like, where $f^{\theta}(x')_k = f^{\theta}(x)_k =c$ with $k=argmax_i f^{\theta}(x)_i$}
The intuitive interpretation of such a guarantee is that for the given neural network and input, there does not exist an adversary that can change the explanation that has been give by more than $\delta$ given that it only perturbs the input by amount specified in $T$. This definition gives us a formal measure of certainty about a provided guarantee which is not provided for any other explanation method.\footnote{As far as I am aware up to now.}


\subsection{Certification Against Model Perturbations}

Below, we formally define what it means for a model to be robustly certifiable at a parameter value $\theta$:
\begin{definition} \textbf{\textit{Model-Certified Explanation}} Given a neural network $f^{\theta}$, a test input $x$, a loss function $J$, a compact parameter set $M$ s.t. $\theta \in M$, and an error tolerance $\delta$, we say that an explanation $e$ is model certified iff: 
\begin{align}
    \forall \theta' \in M, \quad || e - \nabla_x J(f^{\theta'}(x)) || \leq \delta
\end{align}
\end{definition}
\JH{I am not sure it can prevent model fooling because M is too broad... Maybe this training contraints the model class M to models with low curvature with smooth geometry?}
As with input certification, model certification of an explanation allows us to formally guarantee that no adversary exists that can change our explanation by more than $\delta$ given that they perturb weights inside of a fixed range $M$. We will model this intuitively as an $\ell_\infty$-norm ball of radius $\epsilon$ around weights. Thus, the guarantee is that the explanation cannot be changed by an adversary who perturbs each weight and bias value by more than $\epsilon$.

\paragraph{Strongly Certifiable Explanations} We say that an explanation $e$ and model $f^{\theta}$ are \textit{strongly} $\delta$-certifiable if we can prove that both Definitions 1 and 2 hold simultaneously, that is: 
$$ \forall \theta' \in M \wedge \forall x' \in T, \quad ||e - \nabla_{x'} (f^{\theta'}(x'))||  < \delta$$

\subsection{Maximally Certifiable Training}

Given a definition of certifiably robust models and explanations, one might be interested in developing a neural network which has maximally robust explanations. To this end, we can define the following optimal regularizers for input explanation robustness for an input $x$:
$$R_{\text{inp}} = \big( J(f^{\theta}(x), y)  + \argmax_{x' \in T} ||\nabla_x J( f^{\theta}(x')) - \nabla_{x'} J( f^{\theta}(x'))|| \big)$$ 
Similarly, we can define the optimal regularizer for model explanation robustness: 
$$R_{\text{mod}} = \big( J(f^{\theta}(x), y)  + \argmax_{\theta' \in M} ||\nabla_x J( f^{\theta}(x')) - \nabla_{x} J( f^{\theta'}(x))|| \big)$$ 
Lastly, given the entire parameter space $\Theta$, we can state the goal of training a neural network that simultaneously has both optimal performance and optimally robust explanations: 
\begin{align}
    \hat{\theta} = \argmin_{\theta \in \Theta} \sum_{i=0}^{n} R_{*}(J, f^{\theta}, x_i, y_i)
\end{align}
where $* \in \{\text{inp}, \text{mod}\}$. We highlight that while this formulation is very similar to minimax optimization structure to the loss typically used for adversarial training, this loss does not invoke a saddle point solution. That is, the two objectives, minimizing the loss and maximizing the explanation risk are not in direct opposition to one another. Thus, the constraint of robust explanations provides a comparatively less stringent constraint on learning. 

\section{GradCert Algorithms}

In this section, we present methodology for computing explanations that have formal guarantees satisfying Definition 1 and Definition 2.

Our methodology for computing input-certified and model-certified explanations, relies on computing \textit{over-approximations}. Consider, without loss of generality, an input set $T$. An over-approximate gradient set $G$ is one for which we know that $\forall x \in T, \nabla_{x} J( f^{\theta}(x)) \in G$. We can then reason about $G$ in order to ensure that Definition 1 is met. Below, we give a simple procedure for ensuring computing over-approximations of reachable gradients given input perturbation sets and model perturbation sets. 

\subsection{Propagating Input Perturbations}

The key observation we make is that computing an over-approximate gradient set $G$ requires us to maintain an over-approximate output for each operation considered in a forward and backward pass through a neural network (Equations 1-6). The primary operations that we must over approximate are the matrix multiplications (Equations 2 and 4) as well as the application of a non-linear activation function and computation of its derivative (Equation 3 and 4).

We start below stating a lemma that allows us to  over-approximate the result of a matrix multiplication: 

\begin{lemma} Given a matrix $A \in \mathbb{R}^{a \times b}$ and an interval over matrices $B^{L}, B^{U} \in \mathbb{R}^{b \times c}$ s.t. $\forall i,j$ it holds that $B^{L}_{i,j} \leq B^{U}_{i,j}$ we first define the center and radius of the matrix interval w.l.o.g. as $B^{\mu} = (B^{L} + B^{U})/2$ and $B^{r} = (B^{U} - B^{L})/2$. We then have the following inequalities $\forall B^* \in [B^{L}, B^{U}]$:
\begin{align}
    \forall i,j \quad AB^{\mu}_{i,j} - M^{B}_{i,j}  \leq AB^*_{i,j}  \leq AB^{\mu}_{i,j}  + M^{B}_{i,j} 
\end{align}
where $M^{B} = A | B^{r} | $. We denote a function that returns these matrix multiplication bounds given the three parameters above as: 
$C^{L}, C^{U} = \mathcal{O}(A, B^{L}, B^{U})$
\end{lemma}
This lemma allows us to propagate an input set $x^{L}, x^{U}$ through Equation 2 of our forward pass thus enabling us to get bounds on the pre-activation of the first layer, $\zeta^(1)$. Given that our activation functions are monotonic, getting bounds on the activation value is as simple as passing the pre-activation bounds through the activation function. For nearly all practically used activation functions this condition holds. Unfortunately, monotonicity does not hold for the softmax function. However, we can define functions $\sigma_c^{\text{min}}$ and $\sigma_c^{\text{max}}$ that return the minimum and maximum softmax probabilities for class $c$ given bounds on the logit values $z_{l}^{L}, z_{l}^{U}$ (which can be computed using Lemma 1):
\JH{When $x_{min}$ has $c_1=5, c_2=15, c_3=7$, while $x_{max}$ has $c_1=6, c_2=4, c_3=2$ then should $\nabla_{x_{min}} J( f^{\theta}(x_{min}))$ and $\nabla_{x_{max}} J( f^{\theta}(x_{max}))$ be the same? Here their maximum class is different ($c_2$ for $x_{min}$, $c_3$ for $x_{max}$), and the model think $x_{min}$ is close to $c_3$ than $c_1$ while the opposite on $x_{max}$. As XAI should show information of the model prediction on a input, making $\nabla_{x_{min}} J( f^{\theta}(x_{min}))$ and $\nabla_{x_{max}} J( f^{\theta}(x_{max}))$ the same can lead to too insensitive XAI??} \MW{Hm, I think I might be missing something in the question! So here you are refering to $x_{min}$ and $x_{max}$ but I think you are meaning to refer to the outputs $y_{min}$ and $y_{max}$. In this case we know for sure that $y_{min} < y_{max}$  for all class entries and that they consititute an ``over-approximation." But lets chat about this in our next meeting because I think I might misunderstand your question!}
\begin{align}\label{eq:softmaxminimum}
    \sigma^{\text{min}}_c(f, x) &= \dfrac{exp(z_{l,c}^{L})}{exp(z_{l,c}^{L}) + \sum_{k\neq c}exp(z_{l,k}^{U}) } \\
    \sigma^{\text{max}}_c(f, x) &= \dfrac{exp(z_{l,c}^{U})}{exp(z_{l,c}^{U}) + \sum_{k\neq c}exp(z_{l,k}^{L}) } 
\end{align}
Finally, given each of these approximations we can use the resulting worst-case softmax probability bounds and Lemma 1, we can over approximate a backwards pass to compute an over-approximate gradient set. We detail these equations in Algorithm 1.
\footnote{This requires all of the partial derivatives of our activation functions to be monotonic. This is not the case for sigmoid or tanh, however, bounding the partial derivative of these functions between two given points is trivial. This bound/assumption is also necessary for the model-perturbation result below.}

\subsection{Propagating Model Perturbations}

\begin{lemma} Given an interval over matrices $A^{L}, A^{U} \in \mathbb{R}^{a \times b}$ s.t. $\forall i,j$ it holds that $A^{L}_{i,j} \leq A^{U}_{i,j}$, and an interval over matrices $B^{L}, B^{U} \in \mathbb{R}^{b \times c}$. We again take the center and radius of the matrix interval w.l.o.g. as $B^{\mu} = (B^{L} + B^{U})/2$ and $B^{r} = (B^{U} - B^{L})/2$. We also recall that $M^{B} = A|B^{r}|$ and correspondingly, $M^{B} = |A^{r}|$ We then have the following inequalities $\forall A^* \in [A^{L}, A^{U}]$ and $\forall B^* \in [B^{L}, B^{U}]$:
\begin{align}
    \forall i,j \quad &A^{\mu}B^{\mu}_{i,j} - M^{B}_{i,j} - M^{A}_{i,j} - Q_{i,j}   \\ \leq  &A^*B^*_{i,j} \\ \leq  &A^{\mu}B^{\mu}_{i,j} + M^{B}_{i,j} + M^{A}_{i,j} + Q_{i,j}
\end{align}
where $Q = |A^{r}| | B^{r} | $. We denote a function that returns these matrix multiplication bounds given the three parameters above as: 
$C^{L}, C^{U} = \mathcal{O}(A^{L}, A^{U}, B^{L}, B^{U})$
\end{lemma}


\begin{figure}
\centering
\begin{minipage}{.48\textwidth}
  \begin{algorithm}[H]
    %\centering
    \caption{Inp. Grad. Cert.  (ReLu FCNs)}\label{algorithm}
    \textbf{Input:} An $l$-layer neural network $f$, parameters $\theta := \{W_i, b_i\}_{i=0}^{l}$, activation functions $\{\sigma_i\}_{i=0}^{l}$,  an input $x$, an $\ell_\infty$ radius $\epsilon$, an output $y$, and a loss function $\mathcal{L}$ \\
     \textbf{Output:} An explanation $e$, and a robustness guarantee for all inputs in the $\ell_\infty$ ball. 
     \algrule
    \begin{algorithmic}[1]
        \State \text{\# Forward Pass}
        \State $z^{L}_{0} = x - \epsilon$
        \State $z^{U}_{0} = x + \epsilon$
        \State $I^L = \{\}; I^U = \{\}$
        \For{$i \in 0 ... l$}
            \State $\zeta^{L}_{i}, \zeta^{U} = \mathcal{O}(W_i, z^{L}_{0}, z^{U}_{0}, b_i)$
            \State $z^{L}_{i+1} = \sigma_i (\zeta^{L}_{i})$
            \State $z^{U}_{i+1} = \sigma_i (\zeta^{U}_{i})$
            \State $I^L \bigcup z^{L}_{i+1}; I^U \bigcup z^{U}_{i+1}$
        \EndFor
        \State \text{\# Over-approximate softmax}
        \State $y^{L} = \sigma_c^{\text{min}}(z^{L}_{l}, z^{U}_{l})$
        \State $y^{U} = \sigma_c^{\text{max}}(z^{L}_{l}, z^{U}_{l})$
        \State \text{\# Backwards Pass}
        \State $\partial z^{L}_{l} = y - y^{L}$
        \State $\partial z^{U}_{l} = y - y^{U}$
        \For{$i \in 0 ... l$}
            \State $\partial \zeta^{L}_{l-i}, \partial \zeta^{U}_{l-i} = \mathcal{O}(W_{l-i}, \partial z^{L}_{l}, \partial z^{U}_{l})$
            \State $\partial z^{L}_{l-i-1} = \partial \zeta^{L}_{l-i} \cdot sgn(I^L_{l-i}) $
            \State $\partial z^{U}_{l-i-1} = \partial \zeta^{U}_{l-i} \cdot sgn(I^U_{l-i}) $
        \EndFor
        %\State $e = z^{L}_{0} + z^{U}_{0}/2$
        %\State $g = z^{L}_{0} - z^{U}_{0}/2$
        \State \text{return} $z^{L}_{0} + z^{U}_{0}$
    \end{algorithmic}
\end{algorithm}
\end{minipage}%
\hfill
\begin{minipage}{.48\textwidth}
  \centering
  \begin{algorithm}[H]
    %\centering
    \caption{Inp. Grad. Cert.  Training}\label{algorithm}
    \textbf{Input:} An $l$-layer neural network $f$, parameters $\theta := \{W_i, b_i\}_{i=0}^{l}$, activation functions $\{\sigma_i\}_{i=0}^{l}$,  a dataset $\mathcal{D}$, an $\ell_\infty$ radius $\epsilon$, an output $y$, and a loss function $\mathcal{L}$ \\
     \textbf{Output:} A trained NN with maximally robust explanations.
     \algrule
    \begin{algorithmic}[1]
        \While{\textit{Not Converged}}
            \State $(x_i, y_i) \sim \mathcal{D}$
        \EndWhile
    \end{algorithmic}
\end{algorithm}
\end{minipage}
\end{figure}


\subsection{Algorithms for Certifiable Explanations}




 
